Score-Based Generative Classifiers

The tremendous success of generative models in recent years raises the question whether they can also be used to perform classification. Generative models have been used as adversarially robust classifiers on simple datasets such as MNIST, but this robustness has not been observed on more complex datasets like CIFAR-10. Additionally, on natural image datasets, previous results have suggested a trade-off between the likelihood of the data and classification accuracy. In this work, we investigate score-based generative models as classifiers for natural images. We show that these models not only obtain competitive likelihood values but simultaneously achieve state-of-the-art classification accuracy for generative classifiers on CIFAR-10. Nevertheless, we find that these models are only slightly, if at all, more robust than discriminative baseline models on out-of-distribution tasks based on common image corruptions. Similarly and contrary to prior results, we find that score-based are prone to worst-case distribution shifts in the form of adversarial perturbations. Our work highlights that score-based generative models are closing the gap in classification accuracy compared to standard discriminative models. While they do not yet deliver on the promise of adversarial and out-of-domain robustness, they provide a different approach to classification that warrants further research.

==> old_text.tex <==
%Training a classification model on one data distribution and testing it on a different data distribution is still an open problem.
%Biological perception systems are much better in this setting of out-of-distribution (OOD) generalization.
%One hypothesis to explain their success in adapting to new input distributions is that they perform inference in a (hierarchical) generative model of their inputs \citep{rao1999predictive}.
%To turn this generative model into a classifier, the predicted label would be the conditioning variable that maximizes the likelihood of an input $p(x|y)$ under this generative model.
%In contrast, modern machine learning classifiers model the conditional distribution over labels given some input $p(y|x)$, these are commonly referred to as discriminative classifiers.



\begin{comment}
\section{Related Work}
Evaluating generative classifiers
\begin{itemize}
    \item Defense-GAN, ABS, 
    \item Resisting adversarial attacks using gaussian mixture variational autoencoders
    \item Generative Classifiers as a Basis for Trustworthy Image...
    \item Do Deep Generative Models Know What They Don't
    \item UNDERSTANDING THE LIMITATIONS OF CONDITIONAL
GENERATIVE MODELS
\end{itemize}

ScoreBased SDEs literature
\begin{itemize}
    \item ScoreBased SDEs
GENERATIVE MODELS
\end{itemize}
\end{comment}

One proposed explanation for the vulnerability of generative classifiers to adversarial perturbations is based on the observation that generative models are often unable to detect inputs outside the training distribution \citep{nalisnick2018deep,fetaya2019understanding}, although OOD detection based on dataset complexity is one solution to this issue \citep{nalisnick2019detecting}.
Here, we find one source for this behavior but we also demonstrate that our model behaves better in the interpolation experiment.
Yet, we find adversarial perturbations and so, this explanation has to be ruled out for the failure of our SBGC model to generalize to worst case distribution shifts.

In summary, our contributions are:
\begin{itemize}[leftmargin=*]
    \item Using our SBGC model, we report state-of-the-art classification accuracy for generative models on CIFAR-10 \citep{krizhevsky2009learning}, along with highly competitive likelihood values.
    %
    %\item On the common image corruption benchmark CIFAR-10-C \citep{hendrycks2019benchmarking}, we achieve better classification accuracy compared to baseline methods that also do not rely on heavy data augmentations or adversarial training.
    %
    \item Nonetheless, we find that score-based generative classifiers show only slight improvements, if at all, in out-of-of-domain benchmarks and are vulnerable to adversarial examples.
    %\item Lastly, we find that while score-based generative classifiers are not fooled by transfer adversarials, they are fooled by gradient-based attacks (contrary to previous findings \citep{yoon2021adversarial}).
    %(possibly hinting at different inference strategies than discriminative models)
    %\item Additionally, we find that likelihoods increase with different corruptions based on image blurs, which we relate to an underappreciated aspect of modeling natural images.
    %\item adversarial purification paper (https://arxiv.org/pdf/2106.06041.pdf) claimed adversarial robustness when using SDE based models or purification (projection onto image manifold). However, this is not robust (we still need to show this). This happened analogously before in the MNIST literature (DefenseGAN for purification broken in obfuscated gradient paper). However, here an ABS approach was successful. Thus, we investigate ABS approach. We show that it is (not) robust (ongoing experiment). 
    %\item Further experiments: OOD detection; Calibration; Distal adversarials; Nalisnick experiment (train on cifar but test on svhn); Shortcut learning?
\end{itemize}


%While previous work used separate models to parameterize the data distribution of each class individually \citep{schott2018towards}, we find that for score-based generative classifiers models whose score function is conditioned on the class label train more stably and are less prone to overfitting. 
%where $x(0)=x$ and $x(T) = x(0) +  \int_0^T f(x(t), t, y) dt$ is the output of the ODE solver, $p_y(x)$ is the likelihood of $x$ under the model with the score function receiving label $y$ as additional input and $p_\mathrm{prior}$ is a multidimensional normal prior \cite{song2020score}.
%We also test learning another additional scaling on the output of all models $(p_{y=0}(x), \ldots, p_{y=9}(x)) \in \R^{10}$ as suggested by \citet{schott2018towards} to obtain normalized class probabilities after an additional softmax function.
%Similarly, as in this previous work we also tested learning completely separate models without any weight sharing, i.e. $p_y(x) = f_y(x, t)$ which means using a separate score model for each class.

%Restricting the NLL estimation to the correct label $y$ for each sample $\textbf{x}$ further increases the NLL to approximately $3.09 bits/dim.$ (see Appendix XXX), but these conditional likelihoods are not a fair comparison.

%special case of out-of-distribution data. 
%In a first step we test whether adversarial examples of feedforward classifiers transfer to our SBGC and cause prediction errors. We use ??? \citep{huang2019enhancing} to find adversarial 
%In a second step, we directly target our SBGC and compute adversarial input perturbations for this model.

%We evaluate three different settings for the precision of the likelihood inference:
%(1) A precise model, with the Runge-Kutta 45 solver and with absolute and relative precision equal to $10^{-5}$, and the final likelihood averaged over $10$ draws for the epsilon trace estimator.
%(2) A fast model, with the Runge-Kutta 23 solver and with absolute and relative precision equal to $10^{-1}$, and the final likelihood averaged over $10$ draws for the epsilon trace estimator.
%(3) A very fast model, with the same precision and solver as the fast model, but only one epsilon draw for the trace estimator.

%ToDo(check if we can break the previous defense based on ScoreSDEs \citep{yoon2021adversarial})


%To better understand the shortcomings of our SBGC model, we perform the same interpolation experiments.
%Moreover, we analyze the behavior of our SBGC model when challenged with linear interpolations of images. 
%This experiment was previously conducted by \citet{fetaya2019understanding} for some generative models; they found that the likelihood of an interpolated image on CIFAR-10 was actually higher than the likelihoods of both the start $x_A$ and endpoint $x_B$ of the interpolation.

% we do exclude previously suggested explanations by showing that interpolating between images produces convex likelihood curves (Figure~\ref{fig:interpolation_experiment}).
